ANTNets: Mobile Convolutional Neural Networks for Resource Efficient Image Classification

Deep convolutional neural networks have achieved remarkable success in computer vision. However, deep neural networks require large computing resources to achieve high performance. Although depthwise separable convolution can be an efficient module to approximate a standard convolution, it often leads to reduced representational power of networks. In this paper, under budget constraints such as computational cost (MAdds) and the parameter count, we propose a novel basic architectural block, ANTBlock. It boosts the representational power by modeling, in a high dimensional space, interdependency of channels between a depthwise convolution layer and a projection layer in the ANTBlocks. Our experiments show that ANTNet built by a sequence of ANTBlocks, consistently outperforms state-of-the-art low-cost mobile convolutional neural networks across multiple datasets. On CIFAR100, our model achieves 75.7% top-1 accuracy, which is 1.5% higher than MobileNetV2 with 8.3% fewer parameters and 19.6% less computational cost. On ImageNet, our model achieves 72.8% top-1 accuracy, which is 0.8% improvement, with 157.7ms (20% faster) on iPhone 5s over MobileNetV2.

==> blocks.tex <==
\textcolor{red}{Our AntNet is composed of a sequence of ANTBlocks. We replace our ANTBlocks with
different kinds of blocks to see the computational efficiency. As depthwise
kernel $5\times5$ is not as source-efficient as two connected depthwise kernel
$3\times 3$, we always use two depthwise kernel $3\times 3$ for achieving
depthwise kernel $5 \times 5$. The MACCs of depthwise kernel $5 \times 5$
(denoted as $C_5$ )and two connected depthwise kernel $3 \times 3$ (denoted as
$\tilde{C}_5$ ) with the given input $H \times W \times C$ can be calculated
respectively as,}
\begin{align} \label{eq:c23}
C_5 &= H\times W \times C \times 25 \nonumber\\
\tilde{C}_5 &= H\times W \times C \times 18 \\
C_5 &> \tilde{C}_5 \nonumber
\end{align}
\textcolor{red}{
Two $3\times 3$ depthwise kernel has the same effective field as $5 \times 5$
depthwise kernel and two $3\times 3$ offers less computational cost and
parameter count. That is why we use two $3 \times 3$ depthwise kernel, instead
of one $5 \times 5$ depthwise kernel.
We can replace our ANTBlock with different type of blocks to see the different
performance by only modifying the filter sizes and spatial dimensions throughout
the network for ablation study. For the depthwise layer in ANTBlock, we replace
the kernel $3\times 3$ to extract features $H\times W \times tC$ by using
inception depthwise kernels $1\times 1 (C_1), 3 \times 3 (C_3), 5 \times 5
(\tilde{C}_5)$, denoted as $C_{inc}$. Also, in order to decrease the
computational cost and parameter count of the expansion layer in ANTBlock, we
decrease the expansion factor $t$ to half from the second ANTBlock to see its
performance. The Table \ref{tab:variants} shows the result comparison of our
ANTNet with its variants. It shows that $C_3$ performs better than $C_{inc}$
with the same amount of computational cost and parameter count. To reduce the
computational cost and parameter count of the expansion layer, decreasing the
dimension of the expansion layer hurts the performance a lot.  From the ablation
study, our ANTNet shows the better trade-offs over its modified versions with
respect to accuracy-MACCs.}

\begin{table}[!htbp]
	\centering
%	\resizebox{\columnwidth}{!}{
   \small
	 \def\arraystretch{1.2}%
		\begin{tabular} {|c|c|c|c|c|}
			\hline
			Expansion   & Depthwise & \multirow{2}{*}{Top-1 Accu.} & \multirow{2}{*}{\#MAdds} &\multirow{2}{*}{\#Params} \\
			Factor $t$  &  Kernel   &             &         & \\ \hline
			$t = 6$ &  $C_{inc}$  & $74.3$  & $2.2M$ & $73.2M$\\
			$t = 3$ &  $C_3$ & $73.5$ & $1.6M$ & $51.4M$\\
			$t = 3$ &  $\tilde{C}5$ & $73.8$ & $1.7M$ & $55.2M$\\
			$t = 6$ &  $C_3$ & $75.7$ & $2.2M$ & $73.2M$\\
			\hline
		\end{tabular}
%	}
	\caption{\label{tab:variants} \small Performance results of ANTNet and its variants on CIFAR100. }
\end{table}


==> implementation.tex <==
%For production deployment, we have a monolithic implementation that directly access the respective channels for channel-wise attention and group-wise convolution.
For prototyping or experimental reproduction, the channel-wise attention and
group convolution can be implemented using built-in components. Channel-wise
attention can be equivalently implemented as 1x1 regular convolution and group
convolution can be done with the build-in implementation on deep learning
platform, such as Pytorch, or Caffe. 


==> model600.tex <==
{\color{red} To show the representation power of AntBlock, we build larger CNN with $~600$ MAdds budget and compare with those baseline model with similar complexity. There are two ways to build larger CNN, one is to increase the dimension of features with depth multiplier ($\alpha$); another way is to ensemble AntBlock, e-ANTBlock, by mixing AntBlock($g=1$) and AntBlock($g=2$). In order to reach $~600$ MAdds budget, we increase the dimension of each layer of AntNet ($g=2$) by multiplying $\alpha = 1.4$. The performance of this AntNet$^{\star}$ can be seen in Table \ref{tab:antnet} and it offers the highest accuracy of those models with similar complexity, $0.3\%$ Top-1 accuracy higher than MobileNetV2(1.4), $1\%$ Top-1 accuracy higher than NASNet-A and $2\%$ Top-1 accuracy higher than DARTS. By mixing with AntBlock($g=1$) and AntBlock($g=2$), we can have a model, e-AntNet, with $~600$ MAdds budget. The weights $w_1, w_2$ are importance ratio used to weighted those blocks respectively. Both $w_1$ and $w_2$ are scalar variables, which have $w_1 + w_2 = 1, w_1 \geq 0, w_2 \geq 0$. Each $w_1, w_2$ is computed by using a softmax function with $\lambda_1, \lambda_2$ as the controled parameters, which can be learned by back propagation. Table \ref{tab:antnet} shows the favorable performance of AntBlock ensemble (mixture).}
